Projection-Based Constrained Policy Optimization

We consider the problem of learning control policies that optimize a reward function while satisfying constraints due to considerations of safety, fairness, or other costs. We propose a new algorithm, Projection-Based Constrained Policy Optimization (PCPO). This is an iterative method for optimizing policies in a two-step process: the first step performs a local reward improvement update, while the second step reconciles any constraint violation by projecting the policy back onto the constraint set. We theoretically analyze PCPO and provide a lower bound on reward improvement, and an upper bound on constraint violation, for each policy update. We further characterize the convergence of PCPO based on two different metrics: $\normltwo$ norm and Kullback-Leibler divergence. Our empirical results over several control tasks demonstrate that PCPO achieves superior performance, averaging more than 3.5 times less constraint violation and around 15\% higher reward compared to state-of-the-art methods.

==> introduction.tex <==
% !TEX root = iclr2020_SafeRL.tex
\section{Introduction}
%Introduce the problem
In the context of reinforcement learning (RL)
we address the problem of 
%finding 
learning control policies that optimize a reward function while satisfying constraints. For example, these constraints may come from considerations of safety, fairness, cost, or a constraint on some auxiliary variables. Recently, deep RL has demonstrated superior performance on many tasks including the game of  Go~\citep{silver2017mastering}, robotic control~\citep{levine2016end}, and the real time game StarCraft~\citep{openai2019go}.
%
In these tasks the agents are allowed to explore the state space and experiment with every action during training.
However, in many realistic applications such as self-driving cars, unmanned aerial vehicles, and personalized robotic assistants, considerations of safety, fairness and cost (among others) prevent the agent from having the freedom to explore the full environment. 
In effect, the agent is constrained to take actions that ensure the invariance of specified set of desired state-action pairs.  
%
%Consider, for example, an autonomous vehicle learning to cross a junction. 
% Peter's:
%Safety considerations, 
%prevent the vehicle from taking actions that could cause harm to pedestrians or to visits states that result in damage to property (including itself).
%A natural way to incorporate such constraints is by formulating a constrained optimization problem.
%Safety considerations prevent the vehicle from taking actions that could cause harm to pedestrians or 
%
%visiting states that result in damage to property (including itself).


%Review for the other works
%\parab{Related work.}


The problem of learning constraint-satisfying policies is challenging since we need to ensure constrain satisfaction throughout the learning and provide provable guarantees, especially for the robot that learns in the real world.
%
To ensure that every policy update is constraint-satisfying, a natural way to incorporate constraints is by formulating a constrained optimization problem.
%
There have been several 
recent investigations of this problem.
%
For example, \citet{achiam2017constrained} formulated the problem as a constrained optimization problem, and performed policy updates using a conditional gradient approach with line search to ensure constraint satisfaction.
%
However, their base optimization problem becomes infeasible when the current policy violates the constraints.
%
Hence a time-consuming recovery method is used to find a constraint-satisfying policy.
%
In contrast, \citet{tessler2018reward} modelled the problem using an unconstrained optimization problem with weighted constraints added to the reward function.
%
Since the weights are hyperparameters that must be tuned,
this approach incurs the cost of hyperparameter tuning.





%
%\citet{thomas2013projected} proposed a natural gradient projection that projects the natural gradient onto the constraint set. 
%
%Empirically, they found that $\normltwo$ norm projection will move away from the optimal solution, and suggested that Kullback-Leibler (KL) divergence projection is preferred.
%
%However, we note that training is unstable when the Fisher information matrix is ill-conditioned or not well-estimated in the high dimensional policy space, and in such contexts one may need $\normltwo$ norm projection.
%

%Preview & theory
%\parab{Contributions.} 
%In order to solve 

To address the above issues, we propose an iterative algorithm to perform policy update subject to constraints.
%
Unlike the one in \citet{achiam2017constrained} doing incremental steps to check constraint satisfaction, and the one in \citet{tessler2018reward} using soft constraint, 
%
we allow the policy to follow reward improvement direction while using projection onto constraints to ensure constraint satisfaction simultaneously for each policy update.
%
%
%Our algorithm is motivated by the \textit{projected gradient descent}, which is commonly used in the context of constrained optimization, and is motivated by our studies of the constrained policy optimization algorithm (CPO)~\citep{achiam2017constrained}.
%
We call our algorithm  ``Projection Based Constrained Policy Optimization'' (PCPO). 
%
It is decomposed of two steps: 
%
first, we optimize a reward function by constraining
Kullback-Leibler (KL) divergence between the new policy and the previous policy; 
second, we ensure that the new policy satisfies constraints by projecting it onto the constraint set.
%

%
We provide performance guarantees for our algorithm.
%
Specifically, we construct
(1) a lower bound on reward improvement for each policy update,
%
and (2) an upper bound on constraint violation for each policy update.
%
We find that if taking a small step for each policy update, the worst-case constraint violation and reward degradation are alleviated.
%
We further analyze two distance measures for projection onto the constraint set.
%
We find that the convergence of PCPO is affected by the singular value of the Fisher information matrix used during training.
%
This observation can prescribe  what projection should be used during training.

% Experiment 
To explore the practicality of PCPO, 
%
and compare it to other algorithms,
%
we test it on two realistic traffic control tasks proposed in~\citet{vinitsky2018benchmarks}:
%
(1) the agent learns to coordinate the traffic lights in the grid-like road network such as Manhattan, and 
(2) the agent learns to control a fleet of autonomous vehicles in a lane-merging traffic bottleneck such as Oakland-San Francisco Bay Bridge.
%
To make a fair comparison to the existing literature,  
%
we also test our algorithm on two artificial tasks proposed in~\citet{achiam2017constrained}:
(3) the agent learns how to collect desired objects while avoiding collecting undesirable objects,
and (4) the agent learns to walk a circle path while avoiding unsafe regions.
%
In all cases, our algorithm achieves comparable or superior performance to state-of-the-art approaches, with averaging 3.66 times less constraint violation and 14.98 \% more reward improvement.
%
PCPO allows us to robustly learn constraint-satisfying policies, and build a step towards reliable deployment of RL. 


% Closing
%The rest of the paper is organized as follows. 
%
%We review the works in Section \ref{sec:related}. 
%
%In Section \ref{sec:model}, we formally introduce our algorithm, 
%
%and give a theoretical understanding of our algorithm.
%
%We give the practical implementation approach,
%
%and discuss the choice of distance functions for projection in Section \ref{sec:implementation}. 
%
%In Section \ref{sec:experiments}, we demonstrate our experiment results.
%
%Finally, we conclude in Section \ref{sec:conclusion}, where we also give plausible extensions and future research directions.
%


